A Machine Learning Pipeline to Examine Political Bias with Congressional Speeches

Computational methods to model political bias in social media involve several challenges due to heterogeneity, high-dimensional, multiple modalities, and the scale of the data. Political bias in social media has been studied in multiple viewpoints like media bias, political ideology, echo chambers, and controversies using machine learning pipelines. Most of the current methods rely heavily on the manually-labeled ground-truth data for the underlying political bias prediction tasks. Limitations of such methods include human-intensive labeling, labels related to only a specific problem, and the inability to determine the near future bias state of a social media conversation. In this work, we address such problems and give machine learning approaches to study political bias in two ideologically diverse social media forums: Gab and Twitter without the availability of human-annotated data. Our proposed methods exploit the use of transcripts collected from political speeches in US congress to label the data and achieve the highest accuracy of 70.5% and 65.1% in Twitter and Gab data respectively to predict political bias. We also present a machine learning approach that combines features from cascades and text to forecast cascade's political bias with an accuracy of about 85%.

==> Ideas.tex <==
\section{Ideas to validate}
\begin{enumerate}
    \item Machine learning models trained on a given social media forum is proven biased - meaning that model trained on Gab work only on Gab posts for example. Can we create a generalized model from openly available datasets that can identify political bias on multiple social media posts? - To prove this we need to show that the model trained on Twitter does not transfer to Gab and vice versa
    \item Do the opposite of the first idea - Can we transfer model trained on one social media to another?
    \item Identify networks in the social media data
    
\end{enumerate}

==> Related-Old.tex <==
\section{Related Work}

Social media produces large amounts of data that can be exploited to extract valuable information containing human interactions. In recent days, people are not shying away from expressing their opinions and beliefs on these platforms. Social media users often use these platforms to convey their stances~\cite{Darwish_Stefanov_Aupetit_Nakov_2020}. There is a rising concern that these social media sites are responsible for foaming political polarization online. During the time of election, polarization can be found in many posts of social media users~\cite{9026882}. Recently most people prefer to consume news online, which can be another source of polarization as people tend to visit news sources which matche their own political leaning~\cite{Garimella2021PoliticalPI}.

Identification of political bias from text has been a growing interest among researchers,  but this can be quite a challenging task.  Bias can often be detected through inflammatory words present in a sentence or speech.  Most of the early approaches detects bias using traditional "bag-of-words" based classifier to focus on word lexicons~\cite{10.5555/3104482.3104544}.  The major obstacle of these approaches is it heavily relies on primary-level lexical information and neglects semantic structure. Several studies have tried to detect bias inducing words~\cite{Spinde2021AutomatedIO} or biased sentences~\cite{10.1145/3184558.3191640} and articles~\cite{chen-etal-2018-learning} and news mediums.~\cite{baly-etal-2018-predicting}.

Few prior works on political bias or ideology detection have explored Neural Network approaches.  Such a method Recurrent Neural Network (RNN) has been used in~\cite{iyyer2014political} to accumulate the political leaning of each word to determine sentence level bias.  Authors in ~\cite{chen-etal-2020-analyzing} introduced an approach to determine bias in multiple levels such as word,  paragraph and discourse level by employing RNN based model.  It is well established that news articles can have political bias of left leaning or right leaning. The work in~\cite{chen-etal-2018-learning} provided a method to generate an article with the same topic but with flipped political leaning using NLP methods.  

Attention based multi-view model focuses on sentences to identify corresponding political ideology~\cite{Kulkarni2018MultiviewMF}.  Few other work studies similar method at the sentence level in~\cite{Ji2017DistantSF} by extracting relations from text and from news article headlines~\cite{gangula-etal-2019-detecting} along with several baseline models like SVM and CNN.


Other than the traditional bag-of-words based models and sentiment analysis approaches, few researchers tried incorporating graphs to represent opinions and ideologies.  A recent work introduced an opinion-aware knowledge graph which infers based on circumstantial information from text and knowledge bases both~\cite{10.5555/3172077.3172399} by using previous background knowledge from graph. TIMME~\cite{osti_10178656} handles heterogeneity of networks formed from social media sites. CNN is a popular deep learning method which has been extended to GCN~\cite{DBLP:conf/iclr/KipfW17} particularly for graphs, GCN performs well due to its operations being based on Laplacian smoothing. By leveraging textual and social information extracted from news articles,  GCN encoded social information from social networks in order to capture political perspective~\cite{li-goldwasser-2019-encoding}. 

%OKE~\cite{DBLP:conf/apweb/XuLCCQW19} also uses a knowledge graph,  along with this information authors also utilize entity words and opinion words from the textual data.
